RF Sensing Security and Malicious Exploitation: A Comprehensive Survey

Radio Frequency (RF) sensing technologies have experienced significant growth due to the widespread adoption of RF devices and the Internet of Things (IoT). These technologies enable numerous applications across healthcare, smart homes, industrial automation, and human-computer interaction. However, the non-intrusive and ubiquitous nature of RF sensing - combined with its environmental sensitivity and data dependency - makes these systems inherently vulnerable not only as attack targets, but also as powerful attack vectors. This survey presents a comprehensive analysis of RF sensing security, covering both system-level vulnerabilities - such as signal spoofing, adversarial perturbations, and model poisoning - and the misuse of sensing capabilities for attacks like cross-boundary surveillance, side-channel inference, and semantic privacy breaches. We propose unified threat models to structure these attack vectors and further conduct task-specific vulnerability assessments across key RF sensing applications, identifying their unique attack surfaces and risk profiles. In addition, we systematically review defense strategies across system layers and threat-specific scenarios, incorporating both active and passive paradigms to provide a structured and practical view of protection mechanisms. Compared to prior surveys, our work distinguishes itself by offering a multi-dimensional classification framework based on task type, threat vector, and sensing modality, and by providing fine-grained, scenario-driven analysis that bridges theoretical models and real-world implications. This survey aims to serve as a comprehensive reference for researchers and practitioners seeking to understand, evaluate, and secure the evolving landscape of RF sensing technologies.

==> Tab/Authen.tex <==
% % \begin{table*}[htp!]
% % \centering
% % \begin{threeparttable}
% % \caption{\textbf{Comparison of RF Sensing-Based Human Authentication Methods}}
% % \begin{tabular}{c c c c c c}
% % \toprule
% % \textbf{Authentication Scheme} & \textbf{Year} & \textbf{RF Technology} & \textbf{Sensing Target} & \textbf{Key Features} & \textbf{Reference} \\
% % \midrule
% % Wi-Auth & 2017 & Wi-Fi & Motion & Wi-Fi-based 2FA & \cite{shah2017wi} \\
% % Multiauth & 2021 & Wi-Fi & Gait/activities & Multi-user auth & \cite{kong2021multiauth} \\
% % Fingerpass & 2019 & Wi-Fi & Finger gesture & Continuous auth for smart homes & \cite{kong2019fingerpass} \\
% % CAUTION & 2022 & Wi-Fi & Gait & Few-shot open-set recognition & \cite{wang2022caution} \\
% % Wi-access & 2018 & Wi-Fi & Motion & 2FA with Wi-Fi & \cite{shah2018wi} \\
% % Multi-WiIR & 2024 & Wi-Fi & Gait & Multi-user identity check & \cite{wei2024multi} \\
% % Wi-Fi-id & 2016 & Wi-Fi & Gait & Early Wi-Fi-based ID & \cite{zhang2016Wi-Fi} \\
% % Wiwalk & 2022 & Wi-Fi & Gait & Dual-user ID & \cite{ou2022wiwalk} \\
% % NeuralWave & 2018 & Wi-Fi & Gait & DL for gait recognition & \cite{pokkunuru2018neuralwave} \\
% % WiDIGR & 2019 & Wi-Fi & Gait & Direction-independent gait ID & \cite{zhang2019widigr} \\
% % GaitSense & 2021 & Wi-Fi & Gait & Ubiquitous gait ID & \cite{zhang2021gaitsense} \\
% % Gate-ID & 2020 & Wi-Fi & Gait & Direction-independent in smart homes & \cite{zhang2020gate} \\
% % WiHF & 2020 & Wi-Fi & Gestures & Gesture and user recognition & \cite{li2020wihf} \\
% % GaitFi & 2022 & Wi-Fi & Gait & Multimodal with vision & \cite{deng2022gaitfi} \\
% % MetaGanFi & 2022 & Wi-Fi & Gait & Cross-domain ID with few-shot learning & \cite{zhang2022metaganfi} \\
% % Wi-Gait & 2023 & Wi-Fi & Gait & Robust passive ID & \cite{jiang2023wi} \\
% % WiWho & 2016 & Wi-Fi & Gait & Person ID in smart spaces & \cite{zeng2016wiwho} \\
% % WiVi & 2022 & Wi-Fi & Gait & Cross-modal fusion for gait & \cite{fan2022wivi} \\
% % freeGait & 2024 & Wi-Fi & Gait & Mitigates non-gait behaviors & \cite{yan2024freegait} \\
% % Wi-PIGR & 2021 & Wi-Fi & Gait & Path-independent gait ID & \cite{zhang2021wi} \\
% % HumanFi & 2019 & Wi-Fi & Gait & RNN-based human ID & \cite{ming2019humanfi} \\
% % Gait-Enhance & 2023 & Wi-Fi & Gait & Robust recognition of complex patterns & \cite{yang2023gait} \\
% % Gaitid & 2020 & Wi-Fi & Gait & Robust gait recognition & \cite{zhang2020gaitid} \\
% % Imfi & 2021 & Wi-Fi & Gait & Cross-modal gait ID & \cite{song2021imfi} \\
% % EvoSense & 2022 & Wi-Fi & Gait & Self-evolving gait ID & \cite{yao2022evosense} \\
% % Wihi & 2020 & Wi-Fi & Gait & DL for identity ID & \cite{ding2020wihi} \\
% % WiCrew & 2022 & Wi-Fi & Gait & Crew ID for cruise ships & \cite{liu2022wicrew} \\
% % XModal-ID & 2019 & Wi-Fi & Gait & Through-wall ID with video & \cite{korany2019xmodal} \\
% % Wii & 2017 & Wi-Fi & Gait & Device-free passive ID & \cite{lv2017wii} \\
% % WiDFF-ID & 2022 & Wi-Fi & Gait & Fast device-free ID & \cite{wu2022widff} \\
% % OpenAuth & 2024 & mmWave & Gait & Open-world user auth & \cite{yang2024openauth} \\
% % mmpalm & 2024 & mmWave & Palm & Palm recognition for auth & \cite{xie2024mmpalm} \\
% % HeartPrint & 2022 & mmWave & Heartbeat & Heartbeat-based multi-user auth & \cite{wang2022heartprint} \\
% % MU-ID & 2020 & mmWave & Gait & Multi-user ID via gait & \cite{yang2020mu} \\
% % WavoID & 2023 & mmWave & Voice & Multi-modal voice auth & \cite{liu2023wavoid} \\
% % Vocalprint & 2021 & mmWave & Voice & Secure voice auth & \cite{li2021vocalprint} \\
% % Wave-for-safe & 2023 & mmWave & Motion & Mutual auth for unmanned vehicles & \cite{yang2023wave} \\
% % mmSign & 2024 & mmWave & Handwritten signature & Few-shot signature verification & \cite{han2024mmsign} \\
% % Mmsense & 2019 & mmWave & Gait & Multi-person detection and ID & \cite{gu2019mmsense} \\
% % GesturePrint & 2024 & mmWave & Gestures & User ID for gesture recognition & \cite{xu2024gestureprint} \\
% % mmHSV & 2023 & mmWave & Handwritten signature & In-air signature verification & \cite{li2023mmhsv} \\
% % MmSafe & 2022 & mmWave & Voice & Voice security verification & \cite{hao2022mmsafe} \\
% % GaitCube & 2021 & mmWave & Gait & DL for gait recognition & \cite{ozturk2021gaitcube} \\
% % IdentityKD & 2024 & mmWave & Gait & Cross-modal knowledge distillation & \cite{shan2024identitykd} \\
% % MN-UIV & 2024 & mmWave & Gait & Multimodal NN for verification & \cite{zhao2024mn} \\
% % Rdgait & 2024 & mmWave & Gait & Gait ID in complex environments & \cite{wang2024rdgait} \\
% % LoGait & 2023 & LoRa & Gait & Long-range gait ID with DTW & \cite{ge2023logait} \\
% % UWB-Auth & 2024 & UWB & Gait & 2FA with UWB & \cite{cao2024uwb} \\
% % RF-Gait & 2022 & RFID & Gait & Environment-independent gait ID & \cite{jiang2022rf} \\
% % RFPass & 2022 & RFID & Gait & Environment-independent gait auth & \cite{chen2022rfpass} \\
% % Au-id & 2019 & RFID & Sequential activities & Auth via sequential motions & \cite{huang2019id} \\
% % RFree-ID & 2018 & RFID & Gait & Unobtrusive ID irrespective of cofactors & \cite{zhang2018rfree} \\
% % \bottomrule
% % \end{tabular}
% % \end{threeparttable}
% % \label{tab:rf_authentication}
% % \end{table*}
% \begin{table*}[htp!]
% \centering
% \renewcommand{\arraystretch}{1.4} % Adjust row spacing
% \setlength{\tabcolsep}{5.3pt} % Adjust column spacing
% \begin{threeparttable}
% \caption{\textbf{Comparison of RF Sensing-Based Human Authentication Methods}}
% \label{tab:rf_authentication}
% \begin{tabular}{c c c c c c}
% \toprule
% \textbf{Authentication Scheme} & \textbf{Year} & \textbf{RF Technology} & \textbf{Sensing Target} & \textbf{Key Features} & \textbf{Reference} \\
% \bottomrule
% Wi-Auth & 2017 & Wi-Fi & Motion & Wi-Fi-based 2FA & \cite{shah2017wi} \\
% Multiauth & 2021 & Wi-Fi & Gait/activities & Multi-user auth & \cite{kong2021multiauth} \\
% Fingerpass & 2019 & Wi-Fi & Finger gesture & Continuous auth for smart homes & \cite{kong2019fingerpass} \\
% CAUTION & 2022 & Wi-Fi & Gait & Few-shot open-set recognition & \cite{wang2022caution} \\
% Wi-access & 2018 & Wi-Fi & Motion & 2FA with Wi-Fi & \cite{shah2018wi} \\
% Multi-WiIR & 2024 & Wi-Fi & Gait & Multi-user identity check & \cite{wei2024multi} \\
% OpenAuth & 2024 & mmWave & Gait & Open-world user auth & \cite{yang2024openauth} \\
% mmpalm & 2024 & mmWave & Palm & Palm recognition for auth & \cite{xie2024mmpalm} \\
% M-Auth & 2022 & mmWave & Respiration & Respiration-based multi-user auth & \cite{wang2022your} \\
% HeartPrint & 2022 & mmWave & Heartbeat & Heartbeat-based multi-user auth & \cite{wang2022heartprint} \\
% WavoID & 2023 & mmWave & Voice & Multi-modal voice auth & \cite{liu2023wavoid} \\
% Vocalprint & 2021 & mmWave & Voice & Secure voice auth & \cite{li2021vocalprint} \\
% Wave-for-safe & 2023 & mmWave & Motion & Mutual auth for unmanned vehicles & \cite{yang2023wave} \\
% mmSign & 2024 & mmWave & Handwritten signature & Few-shot signature verification & \cite{han2024mmsign} \\
% mmHSV & 2023 & mmWave & Handwritten signature & In-air signature verification & \cite{li2023mmhsv} \\
% MmSafe & 2022 & mmWave & Voice & Voice security verification & \cite{hao2022mmsafe} \\
% MN-UIV & 2024 & mmWave & Gait & Multimodal NN for verification & \cite{zhao2024mn} \\
% UWB-Auth & 2024 & UWB & Gait & 2FA with UWB & \cite{cao2024uwb} \\
% RFPass & 2022 & RFID & Gait & Environment-independent gait auth & \cite{chen2022rfpass} \\
% Au-id & 2019 & RFID & Sequential activities & Auth via sequential motions & \cite{huang2019id} \\
% \bottomrule
% \end{tabular}
% \end{threeparttable}

% \end{table*}
\begin{table*}[htp!]
\centering
\renewcommand{\arraystretch}{1.4}
\setlength{\tabcolsep}{5.3pt}
\begin{threeparttable}
\caption{\textbf{Comparison of RF Sensing-Based Human Authentication and Identification Methods}}
\label{tab:rf_auth_id}
\begin{tabular}{c c c c c c c}
\toprule
\textbf{Scheme} & \textbf{Year} & \textbf{RF Technology} & \textbf{Sensing Target} & \textbf{Biometric Type} & \textbf{Type} & \textbf{Key Features} \\
\midrule
% Authentication entries
Wi-Auth \cite{shah2017wi} & 2017 & Wi-Fi & Motion & Behavioral & Authentication & Wi-Fi-based 2FA \\
MultiAuth \cite{kong2021multiauth} & 2021 & Wi-Fi & Gait/activities & Behavioral & Authentication & Multi-user auth \\
FingerPass \cite{kong2019fingerpass} & 2019 & Wi-Fi & Finger gesture & Behavioral & Authentication & Continuous auth for smart homes \\
CAUTION \cite{wang2022caution} & 2022 & Wi-Fi & Gait & Behavioral & Authentication & Few-shot open-set recognition \\
Wi-Access \cite{shah2018wi} & 2018 & Wi-Fi & Motion & Behavioral & Authentication & 2FA with Wi-Fi \\
Multi-WiIR \cite{wei2024multi} & 2024 & Wi-Fi & Gait & Behavioral & Authentication & Multi-user identity check \\
OpenAuth \cite{yang2024openauth} & 2024 & mmWave & Gait & Behavioral & Authentication & Open-world user auth \\
mmPalm \cite{xie2024mmpalm} & 2024 & mmWave & Palm & Behavioral & Authentication & Palm recognition for auth \\
mmFace \cite{xu2022mask} & 2022 & mmWave & Face & Behavioral & Authentication & Liveness-aware face au \\
M-Auth \cite{wang2022your} & 2022 & mmWave & Respiration & Physiological & Authentication & Respiration-based multi-user auth \\
HeartPrint \cite{wang2022heartprint} & 2022 & mmWave & Heartbeat & Physiological & Authentication & Heartbeat-based multi-user auth \\
WavoID \cite{liu2023wavoid} & 2023 & mmWave & Voice & Behavioral & Authentication & Multi-modal voice auth \\
Wave-for-safe \cite{yang2023wave} & 2023 & mmWave & Motion & Behavioral & Authentication & Mutual auth for unmanned vehicles \\
mmSign \cite{han2024mmsign} & 2024 & mmWave & Handwritten signature & Behavioral & Authentication & Few-shot signature verification \\
MN-UIV \cite{zhao2024mn} & 2024 & mmWave & Gait & Behavioral & Authentication & Multimodal NN for verification \\
UWB-Auth \cite{cao2024uwb} & 2024 & UWB & Gait & Behavioral & Authentication & 2FA with UWB \\
RFPass \cite{chen2022rfpass} & 2022 & RFID & Gait & Behavioral & Authentication & Environment-independent gait auth \\
Au-Id \cite{huang2019id} & 2019 & RFID & Sequential activities & Behavioral & Authentication & Auth via sequential motions \\
\midrule
% Identification entries
Wi-Fi-ID \cite{zhang2016wifi} & 2016 & Wi-Fi & Gait & Behavioral & Identification & Early Wi-Fi-based ID \\
WiWalk \cite{ou2022wiwalk} & 2022 & Wi-Fi & Gait & Behavioral & Identification & Dual-user ID \\
WiHF \cite{li2020wihf} & 2020 & Wi-Fi & Gestures & Behavioral & Identification & Gesture and user recognition \\
GaitFi \cite{deng2022gaitfi} & 2022 & Wi-Fi & Gait & Behavioral & Identification & Multimodal with vision \\
WiCrew \cite{liu2022wicrew} & 2022 & Wi-Fi & Gait & Behavioral & Identification & Crew ID for cruise ships \\
XModal-ID \cite{korany2019xmodal} & 2019 & Wi-Fi & Gait & Behavioral & Identification & Through-wall ID with video \\
Wii \cite{lv2017wii} & 2017 & Wi-Fi & Gait & Behavioral & Identification & Device-free passive ID \\
GesturePrint \cite{xu2024gestureprint} & 2024 & mmWave & Gestures & Behavioral & Identification & User ID for gesture recognition \\
GaitCube \cite{ozturk2021gaitcube} & 2021 & mmWave & Gait & Behavioral & Identification & DL for gait recognition \\
LoGait \cite{ge2023logait} & 2023 & LoRa & Gait & Behavioral & Identification & Long-range gait ID with DTW \\
RF-Gait \cite{jiang2022rf} & 2022 & RFID & Gait & Behavioral & Identification & Environment-independent gait ID \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}

==> Tab/Iden.tex <==
\begin{table*}[htp!]
\centering
\renewcommand{\arraystretch}{1.4} % Adjust row spacing
\setlength{\tabcolsep}{5.3pt} % Adjust column spacing
\begin{threeparttable}
\caption{\textbf{Comparison of RF Sensing-Based Human Identification Methods}}
\label{tab:rf_identification}

\begin{tabular}{c c c c c c}
\toprule
\textbf{Identification Scheme} & \textbf{Year} & \textbf{RF Technology} & \textbf{Sensing Target} & \textbf{Key Features} & \textbf{Reference} \\
\bottomrule
Wi-Fi-id & 2016 & Wi-Fi & Gait & Early Wi-Fi-based ID & \cite{zhang2016wifi} \\
Wiwalk & 2022 & Wi-Fi & Gait & Dual-user ID & \cite{ou2022wiwalk} \\
NeuralWave & 2018 & Wi-Fi & Gait & DL for gait recognition & \cite{pokkunuru2018neuralwave} \\
WiDIGR & 2019 & Wi-Fi & Gait & Direction-independent gait ID & \cite{zhang2019widigr} \\
GaitSense & 2021 & Wi-Fi & Gait & Ubiquitous gait ID & \cite{zhang2021gaitsense} \\
Gate-ID & 2020 & Wi-Fi & Gait & Direction-independent in smart homes & \cite{zhang2020gate} \\
WiHF & 2020 & Wi-Fi & Gestures & Gesture and user recognition & \cite{li2020wihf} \\
GaitFi & 2022 & Wi-Fi & Gait & Multimodal with vision & \cite{deng2022gaitfi} \\
MetaGanFi & 2022 & Wi-Fi & Gait & Cross-domain ID with few-shot learning & \cite{zhang2022metaganfi} \\
Wi-Gait & 2023 & Wi-Fi & Gait & Robust passive ID & \cite{jiang2023wi} \\
WiWho & 2016 & Wi-Fi & Gait & Person ID in smart spaces & \cite{zeng2016wiwho} \\
WiVi & 2022 & Wi-Fi & Gait & Cross-modal fusion for gait & \cite{fan2022wivi} \\
freeGait & 2024 & Wi-Fi & Gait & Mitigates non-gait behaviors & \cite{yan2024freegait} \\
Wi-PIGR & 2021 & Wi-Fi & Gait & Path-independent gait ID & \cite{zhang2021wi} \\
HumanFi & 2019 & Wi-Fi & Gait & RNN-based human ID & \cite{ming2019humanfi} \\
Gait-Enhance & 2023 & Wi-Fi & Gait & Robust recognition of complex patterns & \cite{yang2023gait} \\
Gaitid & 2020 & Wi-Fi & Gait & Robust gait recognition & \cite{zhang2020gaitid} \\
Imfi & 2021 & Wi-Fi & Gait & Cross-modal gait ID & \cite{song2021imfi} \\
EvoSense & 2022 & Wi-Fi & Gait & Self-evolving gait ID & \cite{yao2022evosense} \\
Wihi & 2020 & Wi-Fi & Gait & DL for identity ID & \cite{ding2020wihi} \\
WiCrew & 2022 & Wi-Fi & Gait & Crew ID for cruise ships & \cite{liu2022wicrew} \\
XModal-ID & 2019 & Wi-Fi & Gait & Through-wall ID with video & \cite{korany2019xmodal} \\
Wii & 2017 & Wi-Fi & Gait & Device-free passive ID & \cite{lv2017wii} \\
WiDFF-ID & 2022 & Wi-Fi & Gait & Fast device-free ID & \cite{wu2022widff} \\
MU-ID & 2020 & mmWave & Gait & Multi-user ID via gait & \cite{yang2020mu} \\
Mmsense & 2019 & mmWave & Gait & Multi-person detection and ID & \cite{gu2019mmsense} \\
GesturePrint & 2024 & mmWave & Gestures & User ID for gesture recognition & \cite{xu2024gestureprint} \\
GaitCube & 2021 & mmWave & Gait & DL for gait recognition & \cite{ozturk2021gaitcube} \\
IdentityKD & 2024 & mmWave & Gait & Cross-modal knowledge distillation & \cite{shan2024identitykd} \\
Rdgait & 2024 & mmWave & Gait & Gait ID in complex environments & \cite{wang2024rdgait} \\
LoGait & 2023 & LoRa & Gait & Long-range gait ID with DTW & \cite{ge2023logait} \\
RF-Gait & 2022 & RFID & Gait & Environment-independent gait ID & \cite{jiang2022rf} \\
RFree-ID & 2018 & RFID & Gait & Unobtrusive ID irrespective of cofactors & \cite{zhang2018rfree} \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table*}
